Glass-like Caging with Random Planes

The richness of the mean-field solution of simple glasses leaves many of its features challenging to interpret. A minimal model that illuminates glass physics the same way the random energy model clarifies spin glass behavior would therefore be beneficial. Here, we propose such a real-space model that is amenable to infinite-dimensional analysis and is exactly solvable at high and low densities in finite dimension. By joining analysis with numerical simulations, we uncover geometrical signatures of the dynamical and jamming transitions and provides insight into the origin of activated processes. Translating these findings to the context of standard glass formers further reveals the role played by non-convexity in the emergence of Gardner physics.

==> intro.tex <==
#INTRO 1

The hard-sphere (HS) model is one of the simplest and more insightful model of amorphous materials. Since its nature is purely entropic (energy 0 or $\infty$) its thermodynamic properties are directly related to its geometry. And it is precisely its geometrical analysis that allows very detailed numerical computations that would be unachievable by dynamical means.

The “geometrization" of HS configurations can be achieved by different methods. An important example is the Voronoi tessellation \cite{Voronoi1908,Aurenhammer1991} (and its Delaunay dual), in which the space is partitioned accordingly to the position of the closest sphere center. The metric and topological features of the obtained tessellation gives robust signatures of first order liquid-crystal phase transitions \cite{kumar2005voronoi,senthil2005voronoi}.
Another powerful geometrical method consists in the analysis of free volumes \cite{lennard1937critical}, i.e. cavities explored by a single sphere when all others are kept fixed. The study of their typical volume and surface allows direct estimations of the equation of state \cite{hoover1972exact,Speedy1981CavitiesAF} at high density for both the crystal branch \cite{buehler1951,wood1952note,salsburg1962equation} and the amorphous (glass) branch \cite{hoover1979exact,sastry1997,sastry1998free}. 

The random Lorentz gas (RLG) model allows to naturally pursues this second path of reasoning \cite{jin2015dimensional}. In fact it is a model of free volumes of HSs in the simplified case in which fixed spheres (obstacles) are non-interacting and therefore Poisson distributed (which is equivalent to say that we are only keeping pair correlations). The only interacting sphere is the "wanderer" (or tracer) which explores the free volume. This is a first order cavity approximation and can be easily reversed in order to build the system starting from the central “wanderer". Then the obstacles are Poissonly sampled around the origin resulting in a centered free volume (cage). This inversion, usually referred as planting, is practically very useful since it allows to study the system locally in space (whenever the density is high enough that the cages do not percolate) \cite{biroli2021interplay,biroli2022local}.  Moreover this cavity approximation is exact in the large dimension limit $d\to\infty$ and it is solvable by means of mean-field computations \cite{book_2020}. 

This “geometrization" path can be pushed even further if we approximate the planted spherical obstacles by hyperplanes. Then the geometry of the free volumes becomes convex (we call them cells to differentiate them from cages). In this way we obtain a Poisson convex approximation of HS, which we call the hyperplane-RLG model and will the central subject of this letter. In the limit of high density the hyperplane-RLG is identical to the RLG, since cages asymptotically presents flat surfaces. Decreasing the density the discrepancy between RLG cages and cells increases with a net jump at the percolation density, below which only cells remain bounded. Finally in the limit of small density cells follow the Poisson-Voronoi tessellation.

One of the main reason of our interest in this model stems from the exact mathematical results available for finite $d$. In fact the study of hyperplane tessellation is a central theme in the field of stochastic geometry and in particular in the limit of high(low) density the hyperplane-RLG model can be mapped in the so-called Poisson hyperplane tessellation (PHT)\cite{calka_asymptotic_2013}, for which different exact results have been derived, such as the average volume \cite{horrmann_volume_2014} and the average number of vertexes and facets of the cell \cite{kabluchko_angles_2020,kabluchko_expected_2020} for any finite $d$ system. However for intermediate density, no exact finite $d$ results are available, therefore we have resorted to replica mean-field calculations to evaluate the average volume and $d\to\infty$ limit and compared it with finite size numerical simulations.
It is remarkable that for this model the mean-field results perfectly agrees with extrapolations from small dimensions $d=2,3,4,5,6$. 

Finally we have analysed the compression protocol of HS in the hyperplane-RLG model, which brings the equilibrium configurations to jammed ones \cite{maiti2014free,rainone2015}. Since each sphere is replaced by a hyperplane, compression consists in translation of hyperplanes with respect to the origin. And jamming consists of a cell shrinking as a simplex ($d+1$ hyperplanes) to a point. Equivalently the final point is the center of the largest inscribed sphere in the initial equilibrium cell. Thus for every density there exists a one-to-one map of cell into a point, which can be considered the inherent structure of the cell. While this map is univocal (bijective) in the hyperplane-RLG this is not the case in the RLG model. In fact for any given cage of RLG the “cellification" is directly dependent on the choice of the origin, this non-univocity being related to the Gardner transition \cite{kurchan2013}. 

In this letter we firstly introduce the hyperplane-RLG model, deriving it from the RLG. Then we show that the low and high density limit converge to specific PHT models introduced in stochastic geometry and compare their finite $d$ predictions with numerical simulations. Further on we present mean-field results ($d\to\infty$) for the volume of the cell and compare them with finite $d$ extrapolation of numerical simulations and stochastic geometry results. Finally we introduce the mean-field inherent structure protocol for RLG cells and describe the possible implications concerning the Gardner transition and the jamming line.

#INTRO 2

The hard-sphere (HS) model stands out as a highly simplistic yet profound representation of amorphous materials. Due to its purely entropic nature the thermodynamic properties of the HS model are inherently connected to its geometric attributes. Consequently, through a meticulous analysis of its geometry, remarkably detailed computations become possible, surpassing the limitations of thermodynamic approaches.

The process of "geometrizing" hard-sphere (HS) configurations can be accomplished through various methods. One significant approach involves the utilization of Voronoi tessellation (and its associated Delaunay dual) \cite{Voronoi1908,Aurenhammer1991}, where the space is partitioned based on the proximity to the nearest sphere center. The resulting tessellation exhibits metric and topological characteristics that offer reliable indications of first-order phase transitions, such as the liquid-crystal transition.
Another influential geometric method involves the analysis of free volumes \cite{lennard1937critical}, which refers to the cavities explored by an individual sphere when all others are held in a fixed position. By examining the typical volume and surface characteristics of these free volumes, direct estimations of the equation of state \cite{hoover1972exact,Speedy1981CavitiesAF} can be made, particularly at high densities for both the crystal branch \cite{buehler1951,wood1952note,salsburg1962equation} and the amorphous (glass) branch \cite{hoover1979exact,sastry1997,sastry1998free}.

The random Lorentz gas (RLG) model provides a natural framework to explore the aforementioned second approach  \cite{jin2015dimensional}. Specifically, it serves as a model for investigating the free volumes of hard spheres (HSs) in a simplified scenario where the fixed spheres (obstacles) do not interact with each other and are therefore distributed according to a Poisson distribution (which implies retaining only pair correlations). In this model, a sole interacting sphere, known as the "wanderer" or tracer, explores the available free volume. This approximation, referred to as the first-order cavity approximation, can be conveniently reversed, allowing the construction of the system by initially placing the central "wanderer" and then randomly sampling the obstacles according to a Poisson distribution around the it, resulting in a centered free volume or "cage." This inversion technique, commonly known as "planting", proves to be highly practical as it enables the localized study of the system in space, particularly when the density is sufficiently high to prevent the cages from percolating \cite{biroli2021interplay,biroli2022local}. Furthermore, this cavity approximation is exact in the limit of large dimensions ($d\to\infty$) and can be addressed using mean-field computations \cite{book_2020}.

This approach of "geometrization" can be taken further by approximating the planted spherical obstacles with hyperplanes. By doing so, the geometry of the free volumes becomes convex (referred to as cells to distinguish them from cages). This results in a Poisson convex approximation of the hard-sphere system, that we name hyperplane-RLG model, which forms the central focus of this letter. As the density increases, the hyperplane-RLG model converges to the RLG model, since the cages asymptotically exhibit flat surfaces. However, as the density decreases, the discrepancy between the cages of the RLG model and the cells of the hyperplane-RLG model becomes more pronounced, with a distinct transition occurring at the percolation density, below which only cells remain bounded. Ultimately, in the limit of low density, the cells conform to the Poisson-Voronoi tessellation.

Our interest in this model is driven, in part, by the availability of exact mathematical results for finite dimensions $d$. Specifically, the study of hyperplane tessellation is a prominent topic within the realm of stochastic geometry. Notably, in the high (low) density limit, the hyperplane-RLG model can be mapped onto the Poisson hyperplane tessellation (PHT) \cite{calka_asymptotic_2013}, for which various exact results have been derived. These include the average volume \cite{horrmann_volume_2014}, as well as the average number of vertices and facets of the cell \cite{kabluchko_angles_2020, kabluchko_expected_2020}, applicable to any finite $d$ system. However, for intermediate densities, no exact finite $d$ results are available. Hence, we have employed replica mean-field calculations to evaluate the average volume, particularly in the limit as $d\to\infty$, and have compared these results with numerical simulations conducted on finite-size systems.
Significantly, it is noteworthy that the mean-field results for this model exhibit perfect agreement with extrapolations from low dimensions, specifically $d=2,3,4,5,6$.

Lastly, we have examined the compression protocol of hard spheres (HS) within the hyperplane-RLG model, which drives the equilibrium configurations towards jammed states \cite{maiti2014free,rainone2015}. In this model, each sphere is substituted with a hyperplane, and compression involves translating the hyperplanes relative to the origin. Jamming occurs as a cell, in the shape of a simplex (composed of $d+1$ hyperplanes), contracts to a single point. Alternatively, the final point corresponds to the center of the largest inscribed sphere within the initial equilibrium cell. Consequently, for every density, there exists a unique mapping of the cell to a point, which can be considered as the inherent structure of the cell.
It is important to note that while this mapping is unambiguous (bijective) in the hyperplane-RLG model, it is not the case in the RLG model. Specifically, in the RLG model, the "cellification" process of a given cage depends on the choice of the origin. This lack of univocality is associated with the Gardner transition \cite{kurchan2013}.

In this letter, we begin by introducing the hyperplane-RLG model, which is derived from the RLG model. We then show how the low and high density limits of the hyperplane-RLG model converge to specific models in the realm of stochastic geometry, namely the Poisson hyperplane tessellation (PHT) and compare their predictions with numerical simulations. Additionally, we present mean-field results for the volume of the cell in the hyperplane-RLG model in the limit $d\to\infty$, and compare them with extrapolations from numerical simulations and results from stochastic geometry.
Furthermore, we introduce the mean-field inherent structure protocol for cells in the RLG model, and discuss its potential implications concerning the Gardner transition and the jamming line.
